Investigation of triangularity effects on tokamak edge turbulence through multi-fidelity gyrokinetic simulations

This paper uses the gyro-moment (GM) approach as a multi-fidelity tool to explore the effect of triangularity on tokamak edge turbulence. Considering experimental data from an L-mode DIII-D discharge, we conduct gyrokinetic (GK) simulations with realistic plasma edge geometry parameters at $\rho=0.95$. We find that employing ten GMs effectively captures essential features of both trapped electron mode (TEM) and ion temperature gradient (ITG) turbulence. By comparing electromagnetic GK simulations with adiabatic electron GK and reduced fluid simulations, we identify the range of validity of the reduced models. We observe that TEMs drive turbulent heat transport under nominal discharge conditions, hindering accurate transport level estimates by both simplified models. However, when TEMs are absent, and turbulence is ITG-driven, an agreement across the different models is observed. Finally, a parameter scan shows that the positive triangularity scenario destabilizes the TEM, therefore, the adiabatic electron model tends to show agreement with the electromagnetic simulations in zero and negative triangularity scenarios. On the other hand, the reduced fluid simulations exhibit limited sensitivity to triangularity changes, shedding light on the importance of retaining kinetic effects to accurately model the impact of triangularity turbulence in the tokamak edge. In conclusion, our multi-fidelity study suggests that a GM hierarchy with a limited number of moments is an ideal candidate for efficiently exploring triangularity effects on micro-scale turbulence.

==> 05_triangularity_scan.tex <==
\section{Variation of the triangularity}
The triangularity is varied from $\delta = +0.2$ (PT) and $\delta=-0.2$ (NT), keeping the other parameters in Tab. \ref{ch7_tab:DIIID_params}.
Figure \ref{fig:linear_convergence_analysis_NT_vs_PT} presents the results of the instability growth rates from linear simulations.
We see that increasing the triangularity amplifies strongly the TEM growth rates. 
On the other hand, the TEM instability is entirely stabilized in the NT case. 
The baseline parameters of the DIII-D \#186473 discharge at $\rho=0.95$ lie thus on a thin transition region.

In terms of convergence, the linear results show that the \PJ{2}{1} basis overestimates the stability region of the TEM, as observed for the nominal parameters.
The \PJ{4}{2} basis presents a good agreement with the higher resolution cases in the PT case. 
For NT, the stabilization of the TEM is well captured but the ITG growth rate is increased. 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/linear_convergence_analysis_NT_vs_PT.eps}
    \caption{Linear growth rates (top) and frequencies (bottom) of the DIII-D \#186473 discharge at $\rho=0.95$ setting $\delta=-0.2$ (left) and $\delta=+0.2$ (right) with different GM sets: \PJ{2}{1} (blue), \PJ{4}{2} (red), \PJ{8}{4} (yellow), \PJ{16}{8} (purple)}
    \label{fig:linear_convergence_analysis_NT_vs_PT}
\end{figure}

Finally, we report on 



==> dimensions.tex <==
\topmargin=-0.45in      %
%\evensidemargin=0in     %
\oddsidemargin=-0.1in      %
\textwidth=6.8in        %
\textheight=9.2in       %
%\headsep=0.25in         %
\headheight=30.9pt
